A Hybridized Discontinuous Galerkin Method for A Linear Degenerate Elliptic Equation Arising from Two-Phase Mixtures

We develop a high-order hybridized discontinuous Galerkin (HDG) method for a linear degenerate elliptic equation arising from a two-phase mixture of mantle convection or glacier dynamics. We show that the proposed HDG method is well-posed by using an energy approach. We derive ${\it a priori}$ error estimates for the proposed HDG method on simplicial meshes in both two- and three-dimensions. The error analysis shows that the convergence rates are optimal for both the scaled pressure and the scaled velocity for non-degenerate problems and are sub-optimal by half order for degenerate ones. Several numerical results are presented to confirm the theoretical estimates. We also enhance the HDG solutions by post-processing. The superconvergence rates of $(k+2)$ and $(k+\frac{3}{2})$ are observed for both a non-degenerate case and a degenerate case away from the degeneracy. Degenerate problems with low regularity solutions are also studied, and numerical results show that high-order methods are beneficial in terms of accuracy.

==> Abstract.tex <==
\begin{abstract}
We develop a high-order hybridized discontinuous Galerkin (HDG) method for a linear degenerate elliptic equation arising from a two-phase mixture of mantle convection or glacier dynamics.
We show that the proposed HDG method is well-posed by using an energy approach.
We derive {\it a priori} error estimates for the %proposed HDG
  method on simplicial meshes in both two- and three-dimensions.
The error analysis shows that the convergence rates
are optimal for both the scaled pressure and the scaled velocity for non-degenerate problems and 
are sub-optimal by half order for degenerate ones.
 Several numerical results are presented to confirm the theoretical
 estimates. We also enhance the HDG solutions by post-processing.
The superconvergence rates of $(\k+2)$ and $(\k+\frac{3}{2})$ are observed for both a non-degenerate case
 and a degenerate case away from the degeneracy. 
 Degenerate problems with low regularity solutions are also studied,
 and numerical results show that high-order methods are beneficial in terms of
 accuracy. 
\end{abstract}



==> Conclusion.tex <==
\section{Conclusions and future work}
\seclab{Conclusion}
In this paper, we developed numerical methods for both glacier dynamics and mantle convection.
Both phenomena can be described by a two-phase mixture model,
 in which the mixture of the fluid and the solid is described by the porosity $\phi$ 
(i.e., $\phi >0$ implies the fluid-solid two-phase and $\phi=0$ means the solid single-phase region). 
The challenge is when the porosity vanishes because the system degenerates, which make the problem difficult to solve numerically.  
To address the issue, following \cite{arbogast2016linear}, we start by scaling variables to obtain the well-posedness.
Then we spatially discretize the system using the upwind HDG framework. 
The key feature is that we have modified the upwind HDG flux to accommodate the degenerate (one-phase) region. 
When the porosity vanishes, the unmodified HDG system becomes ill-posed
because the stabilization parameter associated with the HDG flux disappears.
For this reason, we introduce the generalized stabilization parameter 
that is composed of the upwind based parameter $\tau=\phimhalf \d$ in the two-phase region and a positive parameter $\tau=\frac{1}{h}>0$ in the one-phase region.
This enabled us to develop a high-order HDG method for a linear degenerate elliptic equation 
arising from a two-phase mixture of both glacier dynamics and mantle convection. 

We have shown the well-posedness and the convergence analysis of our HDG scheme.
The rigorous theoretical results tell us that our HDG method has the convergence rates of $\LRp{\k+1}$ for a non-degenerate case 
and $\LRp{\k+\half}$ for a degenerate case with a piecewise smooth solution. 

 Several numerical results confirm that our proposed HDG method works well for linear degenerate elliptic equations.
For the non-degenerate case, we obtain the $\LRp{\k+1}$ convergence rates of both the scaled pressure $\p$ and the scaled velocity $\ub$ in two dimensions, whereas in three dimensions we observe the convergence rates above $\LRp{\k+\half}$.
For the degenerate case with a smooth solution, the convergence rate of $\LRp{\k+\half}$ is observed for both the scaled pressure $\p$ and the scaled velocity $\ub$.
For the degenerate case with low solution regularity, the convergence rates of the numerical solutions are bounded by the solution regularity, 
but the high-order method still shows a benefit in terms of accuracy. 
For smooth solutions for which the superconvergence property of HDG methods holds,
we can enhance the HDG solutions by post-processing. We have shown that
the post-processed HDG solution converges to the exact solution
faster than the HDG solution.
The convergence rates for the post-processed solutions are approximately $(\k+2)$ for the non-degenerate case, and $(\k+\frac{3}{2})$ for the degenerate case with a smooth solution. 
Through a parameter study, 
we found that using a positive parameter on the one-phase region does not affect the accuracy of a numerical solution.
We also found that $\tau=1/h$ showed slightly better performance in terms of error levels and convergence rates for the degenerate case with smooth solution. 
%We also found that the generalized stabilization parameter showed slightly better performance in terms of error levels than the other single-valued parameters for the degenerate case with low solution regularity.

In order for our proposed method to work in two-phase flows, 
the interfaces between matrix solid and fluid melt need to be identified 
and grids should be aligned with the interfaces.
In other words, the degeneracies are always required to lie on a set of measure zero. 
Note that we do not consider the full set of dynamical equations 
\eqnref{Darcy}, \eqnref{Stokes}, %\eqnref{MassConservation1}, \eqnref{MassConservation2}, 
\eqnref{MassConservation}, \eqnref{Compaction} yet. %case of partially melted regions yet.
We will tackle this challenge in a future work.




==> ErrorAnalysis.tex <==
\section{Error analysis}

\subsection{NOT COMPLETE}
Suppose $(\ub^e,\q^e)$ be a solution of \eqnref{ScaledDegenerateElliptic2} 
and take $\qh^e$ as the trace of $\q^e$ on the mesh skeleton.
Let us define $\Pr \LRp{\ub^e,\q^e,\qh^e} := \LRp{\Pr \ub^e, \Pr\q^e, \Pi\qh^e}$,
where $\Pi$ is the standard $L^2$-projection 
and the others are coupled projections (to be determined).
We define the following errors
\begin{align}
\eub^I &:= \ub^e - \Pr\ub^e, \quad \eub^h := \Pr\ub^e - \ub, \\
\ep^I &:= \q^e - \Pr\q^e, \quad \ep^h := \Pr\q^e - \q, \\
\eph^I &:= \qh^e - \Pi\qh^e, \quad \eph^h := \Pi\qh^e - \qh.
\end{align}
We take the difference between the true solution and the HDG solution in the weak form of \eqnref{LocalSolver} and \eqnref{GeneralGlobalSolver}
\begin{subequations}
\eqnlab{err}
\begin{align}
  \LRp{ \ub^e - \ub,\testv}_\K 
  - \LRp{ \q^e - \q,\phimhalf \Div \LRp{d(\phi) \testv }}_\K
  + \LRa{ \qh^e - \qh, \phimhalf d(\phi) \testv \cdot \nb }_\pK &=0,\\
  \LRp{ \q^e - \q, \test}_\K
  + \LRp{\phimhalf \Div \LRp{d(\phi) (\ub^e - \ub)},\test }_\K
  + \LRa{\phimhalf d(\phi) \LRp{ (\q^e - \q) - (\qh^e - \qh) },\test}_\pK
  & = 0,\\
  \LRa{\jump{\phimhalf d(\phi) \LRp{\ub^e - \ub}\cdot\n + \tau(\q^e - \q) - \tau(\qh^e-\qh)},\mu}_\e &= 0.
\end{align}
\end{subequations}

We rearrange the system in terms of errors 
\begin{subequations}
\eqnlab{err2}
\begin{align}
  \LRp{\eub^h,\testv}_\K 
  - \LRp{\ep^h,\phimhalf \Div \LRp{d(\phi) \testv }}_\K
  + \LRa{\eph^h, \phimhalf d(\phi) \testv \cdot \nb }_\pK &= \nonumber \\
 - \LRp{\eub^I ,\testv}_\K 
  + \LRp{\ep^I ,\phimhalf \Div \LRp{d(\phi) \testv }}_\K
  - \LRa{\eph^I , \phimhalf d(\phi) \testv \cdot \nb }_\pK,\\
  \LRp{\ep^h, \test}_\K
  + \LRp{\phimhalf \Div \LRp{d(\phi) (\eub^h)},\test }_\K
  + \LRa{\phimhalf d(\phi) \LRp{ (\ep^h) - (\eph^h) } ,\test}_\pK
  &= \nonumber \\
  - \LRp{\ep^I , \test}_\K
  - \LRp{\phimhalf \Div \LRp{d(\phi) ( \eub^I)},\test }_\K
  - \LRa{ \phimhalf d(\phi) \LRp{ (\ep^I) - (\eph^I) },\test}_\pK, \\
  \LRa{\jump{\phimhalf d(\phi) \LRp{\eub^h}\cdot\n + \tau(\ep^h) - \tau(\eph^h)},\mu}_\e &= \nonumber \\
  - \LRa{\jump{\phimhalf d(\phi) \LRp{\eub^I}\cdot\n + \tau(\ep^I) - \tau(\eph^I)},\mu}_\e.
\end{align}
\end{subequations}



%% \begin{subequations}
%% \eqnlab{err3}
%% \begin{align}
%% & \LRp{\eub^h,\vb}_\K - \LRp{\phi^{-\half}\Grad\phi \eq^h, \vb}_\K -
%% \LRp{\phi^\half\eq^h,\Div\vb}_\K + \LRa{\sqrt{\phi}\eqh^h, \vb\cdot\n}_\pK = \notag\\
%% &-\LRp{\eub^I,\vb}_\K + \LRp{\phi^{-\half}\Grad\phi \eq^I, \vb}_\K +
%% \LRp{\phi^\half\eq^I,\Div\vb}_\K - \LRa{\sqrt{\phi}\eqh^I, \vb\cdot\n}_\pK, \\
%% &\LRp{\eq^h,\p}_\K - \LRp{\phi\Grad\phi^{-\half}\cdot\eub^h,\p}_\K - \LRp{\phi^\half\eub^h,\Grad\p}_\K + 
%% \LRa{\eub^h\cdot\n + \LRp{\eq^h - \eqh^h},\Pi\LRp{\sqrt{\phi}\p}}_\pK = \notag\\
%% & -\LRp{\eq^I,\p}_\K + \LRp{\phi\Grad\phi^{-\half}\cdot\eub^I,\p}_\K + \LRp{\phi^\half\eub^I,\Grad\p}_\K - 
%% \LRa{\eub^I\cdot\n + \LRp{\eq^I - \eqh^I},\Pi\LRp{\sqrt{\phi} \p}}_\pK \\
%% &- \myred{\LRa{\eub^I\cdot\n,\sqrt{\phi}\p - \Pi\LRp{\sqrt{\phi}\p}}_\pK}, \\
%% &\LRa{\jump{\eub^h\cdot\n + \eq^h},\mu}_\e = -\LRa{\jump{\eub^I\cdot\n + \eq^I},\mu}_\e.
%% \end{align}
%% \end{subequations}

%% Our goal is to design $\LRp{\Pr \ub^e, \Pr\q^e}$ such that all the
%% boundary integrals and volume ones involving derivatives on the right
%% hand sides of \eqnref{err} vanish, except the \myred{red} term. 
%% In particular, we define $\LRp{\Pr \ub^e, \Pr\q^e}$ to satisfy
%% \begin{subequations}
%% \begin{align}
%% (\eub^I, \vb) &= 0, \quad  \forall \vb \in \polyb{k-1}(\K), \\
%% (\eq^I, \p) &= 0, \quad \forall \p \in \poly{k-1}(\K), \\
%% \LRa{ \jump{\eub^I \cdot \n +  \eq^I} , \mu } &= 0, \quad \forall \mu \in \poly{k}(\pK).
%% \end{align}
%% \end{subequations}
%% Existing result \cite{CockburnGopalakrishnanSayas10} show that
%% $\LRp{\Pr \ub^e, \Pr\q^e}$ is optimal. \myblue{However, we cannot
%%   eliminate volume terms as we could for simple elliptic problems. We
%%   cannot put $\phi$ in the definition of the projection either since degeneration will make the projection equation ill-posed!!}. \mythemec{We need a different strategy here!}

%% \subsection{Different approach}

%% Let us define the energy norm for the group variable $\LRp{\ub,\q,\qh}$ as
%% \[
%% \nor{\LRp{\ub,\q,\qh}}_E^2 :=\sum_\K\nor{\ub}_\K^2 + \nor{\q}_\K^2 + \nor{\q-\qh}_{\pK,\sqrt{\phi}}^2.
%% \]
%% We identify the HDG equations \eqnref{LocalSolver}--\eqnref{GeneralGlobalSolver} with the following
%% \[
%% \b\LRp{\LRp{\ub,\q,\qh}; \LRp{\vb,\p,\mu}} = \g
%% \]

%% \begin{lemma}[Coercivity]
%% The bilinear form $\b\LRp{\LRp{\ub,\q,\qh}; \LRp{\vb,\p,\mu}}$ is
%% coercive with unity coercivity constant in the energy norm.
%% \end{lemma}

%% To show continuity, we start with
%% \begin{align*}
%% &\b\LRp{\LRp{\ub,\q,\qh}; \LRp{\vb,\p,\mu}} = \sum_\K \LRp{\ub,\vb}_\K
%%   - \LRp{\q, \phi^{-\half}\Div\LRp{\phi\vb}}_\K +
%%   \LRa{\qh,\sqrt{\phi}\vb\cdot\n}_\pK \\ &+ \LRp{\q,\p}_\K + \LRp{\p,
%%     \phi^{-\half}\Div\LRp{\phi\ub}}_\K + \LRa{\sqrt{\phi}\LRp{\q -
%%       \qh}, \p - \mu}_\pK - \LRa{\sqrt{\phi}\ub\cdot\n,\mu}_\pK\\ &\le
%% \myblue{  \sqrt{\sum_\K\nor{\ub}^2_\K +
%%     \nor{\phi^{-\half}\Div\LRp{\phi\ub}}^2_\K + 2\nor{\q}_\K^2 +
%%     \nor{\q - \qh}_{\pK,\sqrt{\phi}}^2 + \nor{\qh}^2_{H^{\half}\LRp{\pK}} + \nor{\sqrt{\phi}\ub\cdot\n}_{H^{-\half}\LRp{\pK}}^2}} \\
%% &\times \sqrt{\text{similiar norm for }\LRp{\vb,\p,\mu}} \\
%% & \le 
%% \myorange{\sqrt{\sum_\K\nor{\ub}^2_\K +
%%     \nor{\phi^{-\half}\Div\LRp{\phi\ub}}^2_\K + 2\LRp{1+h^{-1}\max{\sqrt{\phi}}}\nor{\q}_\K^2 
%%     + \LRp{1 + 2\max{\sqrt{\phi}}}\nor{\qh}^2_{H^{\half}\LRp{\pK}} + \nor{\sqrt{\phi}\ub\cdot\n}_{H^{-\half}\LRp{\pK}}^2}} \\
%% &\times \sqrt{\text{similiar norm for }\LRp{\vb,\p,\mu}} \\
%% & \le 
%% \myred{\sqrt{\sum_\K2\nor{\ub}^2_\K +
%%     2\nor{\phi^{-\half}\Div\LRp{\phi\ub}}^2_\K + 2\LRp{1+h^{-1}\max{\sqrt{\phi}}}\nor{\q}_\K^2 
%%     + \LRp{1 + 2\max{\sqrt{\phi}}}\nor{\qh}^2_{H^{\half}\LRp{\pK}}}} \\
%% &\times \sqrt{\text{similiar norm for }\LRp{\vb,\p,\mu}} \\
%% &=: \nort{\LRp{\ub,\q,\qh}} \nort{\LRp{\vb,\p,\mu}},
%% \end{align*}
%% where we have used
%% \begin{itemize}
%% \item \myblue{Cauchy-Schwarz inequality}
%% \item \myorange{triangle and inverse inequalities and the fact that $H^\half$-norm is stronger than $L^2$-norm}
%% \item \myred{trace theorem from Arbogast and Taicher}
%% \end{itemize}

%% \begin{lemma}[Continuity]
%% The bilinear form $\b\LRp{\LRp{\ub,\q,\qh}; \LRp{\vb,\p,\mu}}$ is
%% continuous with respect to the norm $\nort{\cdot}$.
%% \end{lemma}

%% Since we desire to show convergence in the norm $\nort{\cdot}$, which
%% is valid for infinite dimensional objects, we also need to show the
%% coercivity of $\b\LRp{\cdot,\cdot}$ with respect to $\nort{\cdot}$. To
%% that end, we note that in finite dimensions, all norms are equivalent.
%% \begin{lemma}
%% The norms $\nor{}_E$ and $\nort{\cdot}$ are equivalent, i.e.:
%% \[
%% c\nort{\LRp{\ub,\q,\qh}} \le \nor{\LRp{\ub,\q,\qh}}_E \le \nort{\LRp{\ub,\q,\qh}}
%% \]
%% \end{lemma}
%% \begin{proof}
%% The right inequality is trivial, but the left is not. We can bound
%% \[
%% \nor{\phi^{-\half}\Div\LRp{\phi\ub}}_\K^2 \le
%% \LRp{\LRp{\max\LRp{\phi^{-\half}\Grad\phi}}^2 + \LRp{\max\LRp{\phi^{\half}}}^2h^{-1}}\nor{\ub}_\K^2,
%% \]
%% by inverse inequality.

%% \mysierp{Todd: can we bound, perhaps with $\nor{q}_\pK^2$,
%% \[
%% a\nor{q}_\pK^2 + d\nor{\qh}^2_{H^{\half}\LRp{\pK}} \le c\nor{\q - \qh}^2_{\pK,\sqrt{\phi}}
%% \]
%% I have not working with fractional Sobolev norm, though I can define it through minimum extension. Since this is finite dimension, we should be able to do so, but I do not know how to proceed!
%% }
%% \end{proof}

%% We are now in the position to show a Strang lemma for our HDG discretization
%% \begin{theorem}
%% \[
%% \nort{\LRp{\ub^e,\q^e,\eval{\q^e}_{\mc{E}}} - \LRp{\ub,\q,\qh}} \le c \nort{\LRp{\ub,\q,\qh} - \LRp{\ub^h,\q^h,\qh^h}}\]
%% where $\LRp{\ub^e,\q^e,\eval{\q^e}_{\mc{E}}}$ is the exact solution (with sufficient regularity on $\q^e$), $\mc{E}$ the mesh skeleton, and $\LRp{\ub^h,\q^h,\qh^h}$ is an arbitrary function in our HDG spaces.
%% \end{theorem}
%% \begin{proof}
%% Straightforward by Galerkin orthogonality, equivalence of norms, coercivity, and continuity.
%% \end{proof}


==> tbmacrosjcp.tex <==
% MY MACROs
%\newcommand{\k}{k}
\newcommand{\gamD}{{\Gamma_D}}

\newcommand{\TODO}[1]{ \fbox{\parbox{3in}{\bf TODO: #1}}}

\newcommand{\grbf}[1] {\mbox{\boldmath${#1}$\unboldmath}}
%\renewcommand{\grbf}[1] {\mathbf{#1}}
\newcommand{\gbf}[1] {\mathbf{#1}}

%\renewcommand{\baselinestretch}{1.08}

\newcommand{\beq} {\begin{equation}}
\newcommand{\eeq} {\end{equation}}
\newcommand{\bdm} {\begin{displaymath}}
\newcommand{\edm} {\end{displaymath}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bde}{\begin{description}}
\newcommand{\ede}{\end{description}}
\newcommand{\bce}{\begin{center}}
\newcommand{\ece}{\end{center}}
\newcommand{\ben} {\begin{enumerate}}
\newcommand{\een} {\end{enumerate}}
\newcommand{\bea} {\begin{eqnarray}}
\newcommand{\eea} {\end{eqnarray}}
\newcommand{\barr} {\begin{array}}
\newcommand{\earr} {\end{array}}
\newcommand{\bean} {\begin{eqnarray*}}
\newcommand{\eean} {\end{eqnarray*}}
\newcommand{\edoc} {\end{document}}
%\newcommand{\And}{\hspace{0.2cm} \mbox{and} \hspace{0.2cm}}
\newcommand{\On}{\hspace{0.2cm} \mbox{on} \hspace{0.2cm}}
%\newcommand{\Or}{\hspace{0.2cm} \mbox{or} \hspace{0.2cm}}
\newcommand{\In}{\hspace{0.2cm} \mbox{in} \hspace{0.2cm}}
%\newcommand{\For}{\hspace{0.2cm} \mbox{for} \hspace{0.2cm}}
\newcommand{\Minimize}{\hspace{0.2cm} \mbox{minimize} \hspace{0.2cm}}
\newcommand{\Maximize}{\hspace{0.2cm} \mbox{maximize} \hspace{0.2cm}}
\newcommand{\SubjectTo}{\hspace{0.2cm} \mbox{subject} \hspace{0.15cm}
            \mbox{to} \hspace{0.2cm}}

\def\etal{{\it et al.~}}

\newcommand{\point}[1] {\ensuremath{\boldsymbol{#1}}}
\newcommand{\vvec}[1] {\ensuremath{\boldsymbol{#1}}}
\renewcommand{\vec}[1] {\ensuremath{\boldsymbol{#1}}}
%\newcommand{\rvec}[1] {\ensuremath{\boldsymbol{\mathrm{#1}}}}
\newcommand{\cvec}[1] {\ensuremath{\boldsymbol{{#1}}}}
\newcommand{\ten}[1] {\ensuremath{\boldsymbol{#1}}}
\newcommand{\tenfour}[1] {\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\comp}[1]{\begin{pmatrix}{ #1 }\end{pmatrix}}
\newcommand{\vv}{\ensuremath{\vec{v}}}
\newcommand{\vr}{\left(\ensuremath{\vec{r}}\right)}
\newcommand{\att}{\left(t\right)}
\newcommand{\tvv}{\ensuremath{\tilde{\vec{v}}}}
\newcommand{\ww}{\ensuremath{\vec{w}}}
\newcommand{\GG}{\ensuremath{\ten{G}}}
\newcommand{\FF}{\ensuremath{\boldsymbol{\mathfrak{F}}}}
\newcommand{\tEE}{\ensuremath{\tilde{\vec{E}}}}
\newcommand{\nn}{\ensuremath{\vec{n}}}
\renewcommand{\SS}{\ensuremath{\ten{S}}}
\newcommand{\tSS}{\ensuremath{\tilde{\ten{S}}}}
\newcommand{\cp}{\ensuremath{{c_p}}}
\newcommand{\cs}{\ensuremath{{c_s}}}
%\newcommand{\tcp}{\ensuremath{{\tilde{c}_p}}}
\newcommand{\tcs}{\ensuremath{{\tilde{c}_s}}}
\newcommand{\Vp}{\ensuremath{{V^e_p}}}
\newcommand{\Vs}{\ensuremath{{V^e_s}}}
\newcommand{\Ss}{\ensuremath{{S^e_s}}}
\newcommand{\nxnx}[1] {\ensuremath{\nn\times\left(\nn\times{#1}\right)}}

\newcommand{\dd}[2] {\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\DD}[2] {\ensuremath{\frac{d {#1}}{d {#2}}}}
\newcommand{\Grad} {\ensuremath{\nabla}}
\newcommand{\Gradv}[1]{\ensuremath{\nabla_{#1}}}
\newcommand{\Div} {\ensuremath{\nabla\cdot}}
\newcommand{\Divv}[1] {\ensuremath{\nabla_{#1}\cdot}}
\newcommand{\Curl} {\ensuremath{\nabla\times}}
\newcommand{\Cten}{\ensuremath{\tenfour{C}}}

%    Notation for an expression evaluated at a particular condition. The
%    optional argument can be used to override automatic sizing of the
%    right vert bar, e.g. \eval[\biggr]{...}_{...}
\newcommand{\eval}[2][\right]{\relax
  \ifx#1\right\relax \left.\fi#2#1\rvert}

\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\Nel} {\ensuremath{{N_\text{el}}}}
\newcommand{\Ned} {\ensuremath{{N_\text{ed}}}}
\newcommand{\De} {\ensuremath{{\mathsf{D}^e}}}
\newcommand{\Dep} {\ensuremath{{\mathsf{D}^{e'}}}}
\newcommand{\Dhat} {\ensuremath{\hat{\mathsf{D}}}}
\newcommand{\Dehat} {\ensuremath{{\hat{\mathsf{D}}^e}}}
\newcommand{\half} {\ensuremath{\frac{1}{2}}}
\newcommand{\IN} {\ensuremath{{\mathcal{I}_N}}}
\newcommand{\INe} {\ensuremath{{\mathcal{I}_{N_e}}}}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mcC}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mi}[1]{\mathit{#1}}
% \newcommand{\mf}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\Oi}[1]{\int_{\mc{D}} #1 \, d\vec{x}}
\newcommand{\TOi}[1]{\int_{0}^T \int_{\mc{D}} #1 \, d\vec{x}dt}
\newcommand{\Ti}[1]{\int_{0}^T #1 \, dt}
\newcommand{\TDei}[1]{\int_{0}^T\int_{\De} #1 \, d\vec{x}dt}
\newcommand{\TDeid}[1]{\int_{0}^T\int_{\De,N} #1 \, d\vec{x}dt}
\newcommand{\Dei}[1]{\int_{\De} #1 \, d\vec{x}}
\newcommand{\DeI}[1]{\int_{D} #1 \, d\vec{x}}
\newcommand{\DeiM}[1]{\int_{\Dhat} #1 \, d\vec{r}}
\newcommand{\DeMd}[1]{\int_{\De,N_e} #1 \, d\vec{x}}
\newcommand{\DeiMd}[1]{\int_{\Dhat,N_e} #1 \, d\vec{r}}
\newcommand{\DeMdN}[1]{\int_{D,N} #1 \, d\vec{x}}
\newcommand{\DeiMdN}[1]{\int_{\Dhat,N} #1 \, d\vec{r}}
\newcommand{\DeiMdNC}[2]{\int_{\Dhat,N_{#2}} #1 \, d\vec{r}}
\newcommand{\pDei}[1]{\int_{\partial \De} #1 \, d\vec{x}}
\newcommand{\pDeiM}[1]{\int_{\partial \Dhat} #1 \, d\vec{r}}
\newcommand{\pDeiMd}[1]{\int_{\partial \Dhat,N_e} #1 \, d\vec{r}}
\newcommand{\pDeiMdN}[1]{\int_{\partial \Dhat,N} #1 \, d\vec{r}}
\newcommand{\pDeiMdNC}[2]{\int_{\partial \Dhat,N_{#2}} #1 \, d\vec{r}}
\newcommand{\pMortar}[2]{\int_{\mc{M}_{#2}} #1 \, d\vec{r}}
\newcommand{\pMortard}[2]{\int_{\mc{M}^{#2},N_{#2}} #1 \, d\vec{r}}
\newcommand{\pMortardd}[3]{\int_{\mc{M}^{#2},N_{#3}} #1 \, d\vec{r}}
\newcommand{\pMortardh}[3]{\int_{\mc{M}_{#2},N_{#3}} #1 \, d\vec{r}}
\newcommand{\pMortardhn}[4]{\int_{{#2}_{#3},N_{#4}} #1 \, d\vec{r}}
\newcommand{\TpDei}[1]{\int_{0}^T\int_{\partial \De} #1 \, d\vec{x}}
\newcommand{\TpDeid}[1]{\int_{0}^T\int_{\partial \De,N} #1 \, d\vec{x}}
\newcommand{\Deid}[1]{\int_{\De,N_e} #1 \, d\vec{x}}
\newcommand{\DeidN}[1]{\int_{\De,N} #1 \, d\vec{x}}
\newcommand{\pDeidN}[1]{\int_{\partial \De,N} #1 \, d\vec{x}}
\newcommand{\pDeid}[1]{\int_{\partial \De,N_e} #1 \, d\vec{x}}
\newcommand{\nor}[1]{\left\| #1 \right\|}
\newcommand{\snor}[1]{\left| #1 \right|}
\newcommand{\LRp}[1]{\left( #1 \right)}
\newcommand{\LRs}[1]{\left[ #1 \right]}
\newcommand{\LRa}[1]{\left< #1 \right>}
\newcommand{\LRc}[1]{\left\{ #1 \right\}}
\newcommand{\pp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppcp}[1]{\frac{\partial #1}{\partial \vec{c_p}}}
\newcommand{\ppcpj}[1]{\frac{\partial #1}{\partial c_p}}
\newcommand{\ppcpmf}[1]{\frac{\partial #1}{\partial \vec{\mf{c_p}}}}
\newcommand{\ppm}[1]{\frac{\partial #1}{\partial \vec{m}}}
\newcommand{\ppho}[3]{\frac{\partial^{#3} #1}{{\partial #2}^{#3}}}
\newcommand{\ppmi}[1]{\frac{\partial #1}{\partial m_i}}
\newcommand{\ppmj}[1]{\frac{\partial #1}{\partial m_j}}
\newcommand{\ppcpm}[1]{\frac{\partial #1}{\partial \vec{c_p}^-}}
\newcommand{\ppcpp}[1]{\frac{\partial #1}{\partial \vec{c_p}^+}}
\newcommand{\ppcs}[1]{\frac{\partial #1}{\partial \vec{c_s}}}
\newcommand{\ppcsm}[1]{\frac{\partial #1}{\partial \vec{c_s}^-}}
\newcommand{\ppcsp}[1]{\frac{\partial #1}{\partial \vec{c_s}^+}}
\newcommand{\td}[2]{\frac{d #1}{d #2}}
\newcommand{\Rvert}[1]{\left. #1 \right|}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\ipDed}[3]{\LRp{ #1, #2}_{\De,N}^{#3}}

\newcommand{\bigO}{\mathcal{O}}
%\newcommand{\supp}{\text{supp}}

\newcommand{\iOm}[1]{\int_{\Omega} #1 \, d\Omega}
\newcommand{\iGb}[1]{\int_{\Gamma_{b}} #1 \, ds}
\newcommand{\iGs}[1]{\int_{\Gamma_{s}} #1 \, ds}
\newcommand{\iGsy}[1]{\int_{\Gamma_{s}} #1 \, ds(\mb{y})}
\newcommand{\RE}{\mbox{{I}}\hspace{-0.5ex}\mbox{{R}}}
\newcommand{\iC}[1]{\int_{0}^{2\pi} #1 \, d\theta}
\newcommand{\iGr}[1]{\int_{\Gamma_{\infty}} #1 \, ds}

\newcommand{\jump}[1] {\ensuremath{[\![{#1}]\!]}}
\newcommand{\diff}[1] {\ensuremath{\LRs{#1}}}
\newcommand{\average}[1] {\ensuremath{\LRc{\!\{#1\}\!}}}

\newcounter{tablecell}

\newcommand*{\numbercell}{%
  \stepcounter{tablecell}%
  \thetablecell. % **
}

\newtheorem{propo}{Proposition}
\newtheorem{coro}{Corollary}
\newtheorem{theo}{Theorem}
\newtheorem{lem}{Lemma}

%\theoremstyle{definition}
\newtheorem{defi}{definition}

%\theoremstyle{remark}
\newtheorem{rema}{remark}

\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\eqnlab}[1]{\label{eq:#1}}
\newcommand{\theolab}[1]{\label{theo:#1}}
\newcommand{\corolab}[1]{\label{coro:#1}}
\newcommand{\propolab}[1]{\label{propo:#1}}
\newcommand{\lemlab}[1]{\label{lem:#1}}
\newcommand{\defilab}[1]{\label{defi:#1}}
\newcommand{\remalab}[1]{\label{rema:#1}}
\newcommand{\tablab}[1]{\label{tab:#1}}

\newcommand{\figref}[1]{\ref{fig:#1}}
\newcommand{\theoref}[1]{\ref{theo:#1}}
\newcommand{\defiref}[1]{\ref{defi:#1}}
\newcommand{\remaref}[1]{\ref{rema:#1}}
\newcommand{\cororef}[1]{\ref{coro:#1}}
\newcommand{\proporef}[1]{\ref{propo:#1}}
\newcommand{\lemref}[1]{\ref{lem:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\alglab}[1]{\label{alg:#1}}
\newcommand{\algref}[1]{\ref{alg:#1}}
\newcommand{\seclab}[1]{\label{sect:#1}}
\newcommand{\secref}[1]{\ref{sect:#1}}
\newcommand{\tabref}[1]{\ref{tab:#1}}

\renewcommand{\u}{u}
\renewcommand{\v}{v}
\newcommand{\un}{\u_h}
\newcommand{\e}{e}
\newcommand{\w}{w}
\newcommand{\wb}{\mb{\w}}
\newcommand{\J}{J}
\newcommand{\Jb}{\mb{J}}
\newcommand{\q}{q}
\renewcommand{\r}{r}
\newcommand{\qh}{\hat{\q}}
\newcommand{\qs}{\q^*}
\newcommand{\qht}{\tilde{\qh}}
\newcommand{\qbar}{\overline{\q}}
\newcommand{\qb}{{\mb{\q}}}
\newcommand{\sig}{{\sigma}}
\newcommand{\thetah}{{\hat{\theta}}}
\newcommand{\thetas}{{\theta^*}}
\newcommand{\thetahn}{{\thetah_h}}
\newcommand{\sign}[1]{\text{ sgn}\!\LRp{#1}}
\newcommand{\sigh}{\hat{\sig}}
\newcommand{\sigs}{\sig^*}
\newcommand{\sigb}{{\bs{\sig}}}
\newcommand{\sigbn}{\sigb_h}
\newcommand{\sigbs}{\sigb^*}
\newcommand{\taub}{{\bs{\tau}}}
\newcommand{\kappab}{{\bs{\kappa}}}
\newcommand{\gamb}{{\bs{\gamma}}}
\newcommand{\ut}{\tilde{\u}}
\newcommand{\sigbt}{\tilde{\sigb}}
\newcommand{\vt}{\tilde{\v}}
\newcommand{\taubt}{\tilde{\taub}}
\newcommand{\ub}{\mb{\u}}
\newcommand{\ubp}{\mb{\u}^+}
\newcommand{\ubm}{\mb{\u}^-}
\newcommand{\vb}{\mb{\v}}
\newcommand{\um}{\u^-}
\newcommand{\up}{\u^+}


\newcommand{\m}{{m}}

\newcommand{\ud}{{\dot{\u}}}
\newcommand{\vd}{{\dot{\v}}}
\newcommand{\sigbd}{{\dot{\sigb}}}
\newcommand{\taubd}{\dot{\taub}}

\renewcommand{\d}{{d}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\kap}{\kappa}
\newcommand{\F}{\mb{F}}
\newcommand{\f}{f}
\newcommand{\g}{g}
\newcommand{\fb}{\mb{\f}}
\newcommand{\gb}{\mb{\g}}
\newcommand{\gD}{g_D}
\newcommand{\pOmega}{\partial \Omega}
\newcommand{\K}{K}
\newcommand{\Kp}{K^+}
\newcommand{\Km}{K^-}
\newcommand{\pK}{{\partial \K}}
\newcommand{\Kj}{{\K_j}}
\newcommand{\Gh}{{\mc{E}_h}}
\newcommand{\Gho}{{\mc{E}_h^o}}
\newcommand{\Ghb}{{\mc{E}_h^{\partial}}}
\newcommand{\Poly}{{{\mc{P}}}}
\newcommand{\D}{{D}}
\newcommand{\p}{{p}}
\newcommand{\Ts}{{\mb{T}}}
\newcommand{\Vb}{{\mb{V}}}
\newcommand{\V}{{V}}
\newcommand{\Lam}{{\Lambda}}
\newcommand{\Lamb}{\bs{\Lambda}}
\newcommand{\mub}{\bs{\mu}}
\newcommand{\lambdab}{\bs{\lambda}}
\newcommand{\Th}{{\Ts_h}}
\newcommand{\Vh}{{\V_h}}
\newcommand{\Vbh}{{\Vb_h}}
\newcommand{\Lamh}{{\Lam_h}}
\newcommand{\Lambh}{{\Lamb_h}}
\newcommand{\Lamho}{{\overline{\Lam}_h}}
\newcommand{\Lambht}{{\Lamb_h^t}}
\newcommand{\Ltwo}{{L^2\LRp{\Omega}}}
\newcommand{\Ltwoe}{{L^2\LRp{\e}}}
\newcommand{\Ltw}{{L^2\LRp{\K}}}
\newcommand{\VhK}{{\V_h\LRp{\K}}}
\newcommand{\ThK}{{\Ts_h\LRp{\K}}}
\newcommand{\VbhK}{{\Vb_h\LRp{\K}}}
\newcommand{\Lamhe}{{\Lam_h\LRp{\e}}}
\newcommand{\Lambhe}{{\Lamb_h\LRp{\e}}}
\renewcommand{\L}{\mc{L}}
\renewcommand{\D}{\mc{D}}
\newcommand{\T}{\mc{T}}
\newcommand{\Tt}{\tilde{\T}}
\newcommand{\A}{\mb{A}}
\newcommand{\B}{\mb{B}}
\renewcommand{\D}{\mb{D}}
\newcommand{\Am}{\A^-}
\newcommand{\Ap}{\A^+}
\newcommand{\Aa}{\snor{\A}}
\newcommand{\Rb}{\mb{R}}
\newcommand{\C}{\mb{C}}
\renewcommand{\S}{\mb{S}}
\newcommand{\Sm}{\S^{-}}
\newcommand{\Sp}{\S^{+}}
\newcommand{\Spm}{\S^{\pm}}
\newcommand{\Q}{\mb{Q}}

\newcommand{\Lte}{{L^2\LRp{\Gh}}}
\newcommand{\n}{\mb{n}}
\newcommand{\nm}{\n^-}
\newcommand{\np}{\n^+}
\newcommand{\uh}{{\hat{\u}}}
\newcommand{\us}{{\u^*}}
\newcommand{\uhn}{{\uh_h}}
\newcommand{\ubh}{{\hat{\ub}}}
\newcommand{\ubs}{{\ub^*}}
\newcommand{\ubht}{{\tilde{\ubh}}}
\newcommand{\uht}{{\tilde{\uh}}}
\newcommand{\uhtn}{{\uht_h}}
\newcommand{\uhd}{{\dot{\uh}}}
\newcommand{\sigbh}{{\hat{\sigb}}}
\newcommand{\Fh}{{\hat{\F}}}
\newcommand{\Fs}{\F^*}
\renewcommand{\c}{{c}}

\newcommand{\zb}{\mb{z}}
\renewcommand{\sb}{\mb{s}}
\newcommand{\rb}{\mb{r}}
\newcommand{\betab}{\bs{\beta}}
\newcommand{\veps}{{\varepsilon}}
\newcommand{\vepsb}{\bs{\veps}}
\newcommand{\Hb}{\mb{H}}
\newcommand{\Hbt}{\Hb^t}
\newcommand{\Eb}{\mb{E}}
\newcommand{\Ebt}{\Eb^t}
\newcommand{\hb}{\mb{h}}
\newcommand{\eb}{\mb{e}}
\newcommand{\Hbh}{\hat{\mb{H}}}
\newcommand{\Ebh}{\hat{\mb{E}}}
\newcommand{\Hbs}{{\mb{H}^*}}
\newcommand{\Ebs}{{\mb{E}^*}}
\newcommand{\Ebht}{\Ebh^t}
\newcommand{\Hbht}{\Hbh^t}
\newcommand{\Lb}{\mb{L}}
\newcommand{\Gb}{\mb{G}}
\newcommand{\Lbh}{\hat{\Lb}}
\newcommand{\Lbs}{\Lb^*}
\newcommand{\Ib}{\mb{I}}
\newcommand{\Sigb}{\bs{\Sigma}}
\newcommand{\Piu}{\Pi_\u}
\newcommand{\Pisigb}{\Pi_\sigb}
\newcommand{\Z}{Z}
\newcommand{\Y}{Y}
%\newcommand{\m}{m}
\newcommand{\rhou}{\rho\u}
\newcommand{\rhov}{\rho\v}
\newcommand{\E}{E}
\renewcommand{\P}{P}
\newcommand{\h}{H}
\newcommand{\diag}{\text{diag}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}[theorem]{Remark}


==> test.tex <==

\section{Test}

%\begin{table}[t]
%\caption{Convergence test for non-degenerate case with smooth solution: triangular elements are used.}
%\label{table-triangle}
%\begin{center}
%\begin{tabular}{*{6}{c}}
%\hline
%\multirow{2}{*}{p} & \multirow{2}{*}{h} 
%& \multicolumn{2}{c}{$\left\Vert p^e - p     \right\Vert _{2}$} 
%& \multicolumn{2}{c}{$\left\Vert {\bf u}^e - {\bf u} \right\Vert _{2}$} \tabularnewline
%  &  &   error & order & error & order \tabularnewline
%\hline\hline
%      &   0.1400 & 6.521E-01 &      $-$ &   5.021E+00 &      $-$ \tabularnewline
%    1 &   0.0700 & 1.813E-01 &    1.847 &   1.436E+00 &    1.806 \tabularnewline
%      &   0.0350 & 4.726E-02 &    1.940 &   3.794E-01 &    1.920 \tabularnewline
%\tabularnewline
%      &   0.1400 & 9.445E-02 &      $-$ &   8.312E-01 &      $-$ \tabularnewline
%    2 &   0.0700 & 1.245E-02 &    2.924 &   1.071E-01 &    2.956 \tabularnewline
%      &   0.0350 & 1.587E-03 &    2.971 &   1.354E-02 &    2.984 \tabularnewline
%\tabularnewline
%      &   0.1400 & 8.929E-03 &      $-$ &   6.658E-02 &      $-$ \tabularnewline
%    3 &   0.0700 & 5.865E-04 &    3.928 &   4.570E-03 &    3.865 \tabularnewline
%      &   0.0350 & 3.728E-05 &    3.976 &   2.942E-04 &    3.957 \tabularnewline
%\tabularnewline
%      &   0.1400 & 8.015E-04 &      $-$ &   7.305E-03 &      $-$ \tabularnewline
%    4 &   0.0700 & 2.571E-05 &    4.963 &   2.292E-04 &    4.995 \tabularnewline
%      &   0.0350 & 8.124E-07 &    4.984 &   7.199E-06 &    4.992 \tabularnewline
%\hline\hline
%\end{tabular}
%\end{center}
%\end{table}


\begin{table}[t]
\caption{Convergence test for degenerate case with smooth solution: upwind based stabilization parameter is used.
BEFORE implies that imposing $\tau=0$ for two-phase region and $\tau=1/h$ for one-phase region at the intersection, 
whereas AFTER implies that imposing both the $\tau=1/h$ for one- and two- phase region at the intersection.}
\label{table-tau}
\begin{center}
\begin{tabular}{*{10}{c}}
\hline
\multirow{2}{*}{p} & \multirow{2}{*}{h}
& \multicolumn{4}{c}{ BEFORE } & \multicolumn{4}{c}{AFTER } \tabularnewline
& 
& \multicolumn{2}{c}{$\left\Vert p^e - p     \right\Vert _{2}$}
& \multicolumn{2}{c}{$\left\Vert {\bf u}^e - {\bf u} \right\Vert _{2}$} 
& \multicolumn{2}{c}{$\left\Vert p^e - p     \right\Vert _{2}$}
& \multicolumn{2}{c}{$\left\Vert {\bf u}^e - {\bf u} \right\Vert _{2}$} \tabularnewline
  &  &   error & order & error & order & error & order & error & order \tabularnewline
\hline\hline
\multirow{4}{*}{ 1}     &   0.1250 &    7.534E-01 &      $-$ &    1.251E+01 &      $-$ &     7.534E-01 &      $-$ &   1.251E+01 &      $-$ \tabularnewline
                        &   0.0625 &    2.187E-01 &    1.784 &    5.714E+00 &    1.130 &     2.188E-01 &    1.784 &   5.714E+00 &    1.130 \tabularnewline
                        &   0.0312 &    7.322E-02 &    1.579 &    2.386E+00 &    1.260 &     7.323E-02 &    1.579 &   2.386E+00 &    1.260 \tabularnewline
                        &   0.0156 &    2.403E-02 &    1.608 &    9.371E-01 &    1.348 &     2.403E-02 &    1.608 &   9.371E-01 &    1.348 \tabularnewline
\tabularnewline                                                                                                                           
\multirow{4}{*}{ 2}     &   0.1250 &    1.003E-01 &      $-$ &    2.911E+00 &      $-$ &     1.004E-01 &      $-$ &   2.911E+00 &      $-$ \tabularnewline
                        &   0.0625 &    1.818E-02 &    2.465 &    5.997E-01 &    2.279 &     1.819E-02 &    2.465 &   5.996E-01 &    2.279 \tabularnewline
                        &   0.0312 &    3.078E-03 &    2.562 &    1.154E-01 &    2.378 &     3.083E-03 &    2.561 &   1.154E-01 &    2.378 \tabularnewline
                        &   0.0156 &    4.895E-04 &    2.653 &    2.080E-02 &    2.472 &     4.907E-04 &    2.651 &   2.080E-02 &    2.472 \tabularnewline
\tabularnewline                                                                                                                           
\multirow{4}{*}{ 3}     &   0.1250 &    1.006E-02 &      $-$ &    2.552E-01 &      $-$ &     1.016E-02 &      $-$ &   2.551E-01 &      $-$ \tabularnewline
                        &   0.0625 &    8.438E-04 &    3.575 &    2.636E-02 &    3.275 &     8.531E-04 &    3.574 &   2.635E-02 &    3.275 \tabularnewline
                        &   0.0312 &    6.780E-05 &    3.638 &    2.542E-03 &    3.374 &     6.857E-05 &    3.637 &   2.542E-03 &    3.374 \tabularnewline
                        &   0.0156 &    5.168E-06 &    3.713 &    2.316E-04 &    3.456 &     5.239E-06 &    3.710 &   2.316E-04 &    3.456 \tabularnewline
\tabularnewline                                                                                                                           
\multirow{4}{*}{ 4}     &   0.1250 &    7.227E-04 &      $-$ &    2.951E-02 &      $-$ &     7.243E-04 &      $-$ &   2.951E-02 &      $-$ \tabularnewline
                        &   0.0625 &    3.676E-05 &    4.297 &    1.717E-03 &    4.103 &     3.700E-05 &    4.291 &   1.717E-03 &    4.103 \tabularnewline
                        &   0.0312 &    1.596E-06 &    4.525 &    8.585E-05 &    4.322 &     1.615E-06 &    4.518 &   8.585E-05 &    4.322 \tabularnewline
                        &   0.0156 &    6.451E-08 &    4.629 &    3.994E-06 &    4.426 &     6.562E-08 &    4.621 &   3.994E-06 &    4.426 \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}


%\subsection{A two-dimensional sine solution test}
%
%Figure \figref{test-2d-tc3-convergece} shows the spatial convergence results using $L^2 (\Omegah)$ 
%by refining the mesh with $n=\{16,32,64\}$ for $\tau=\sqrt{\phi}/h$ and with $n=\{16,32,64,128\}$ for others. We observe that $q$ has the convergence rate of $p+1$ and $u_y$ has that of $p$. 
%Compared to $\tau=\sqrt{\phi}$, multiplying the $1/h$ term so that $\tau=\sqrt{\phi}/h$ seems to enhance convergence rate for $q$, but degrade $u_y$. 
%
%
%  \begin{figure}[h!t!b!]
%    \centering
%% tau = sqrt(\phi)
%    \subfigure[$q$ with $\tau=\sqrt{\phi}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau1-q}
%      \figlab{test-2d-tc3-conv-tau1-q}
%    }
%    \subfigure[$u_x$ with $\tau=\sqrt{\phi}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau1-ux}
%      \figlab{test-2d-tc3-conv-tau1-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\sqrt{\phi}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau1-uy}
%      \figlab{test-2d-tc3-conv-tau1-uy}
%    }
%% tau = 1/h
%    \subfigure[$q$ with $\tau=\frac{1}{h}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau2-q}
%      \figlab{test-2d-tc3-conv-q}
%    }
%    \subfigure[$u_x$ with $\tau=\frac{1}{h}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau2-ux}
%      \figlab{test-2d-tc3-conv-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\frac{1}{h}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau2-uy}
%      \figlab{test-2d-tc3-conv-uy}
%    }
%%tau = sqrt/h
%    \subfigure[$q$ with $\tau=\frac{\sqrt{\phi}}{h}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau4-q}
%      \figlab{test-2d-tc3-conv-tau4-q}
%    }
%    \subfigure[$u_x$ with $\tau=\frac{\sqrt{\phi}}{h}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau4-ux}
%      \figlab{test-2d-tc3-conv-tau4-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\frac{\sqrt{\phi}}{h}$ ]{
%      \includegraphics[trim=.0cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc3-kx2ky3-conv-tau4-uy}
%      \figlab{test-2d-tc3-conv-tau4-uy}
%    }
%
%    \caption{Convergence study with different $\tau$ for the sine solution test ($k_x=2$ and $k_y=3$): scaled pressure $q$, scaled velocity component $u_x$ and scaled velocity component $u_y$ for $\tau=\sqrt{\phi}$, $\tau=1/h$ and $\tau=\sqrt{\phi}/h$. }
%    \figlab{test-2d-tc3-convergece}
%  \end{figure}
%
%
%
%\subsubsection{A smooth solution test in two dimensions}
%
%
%As shown in \figref{test-2d-tc4-convergence}, 
%the convergence rate of $q$ with different $\tau$ is $p+1$ and that of $u_y$ is $p+1/2$. 
%
%
%\begin{figure}[h!t!b!]
%    \centering
%%tau= sqrt(phi)
%    \subfigure[$q$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-q}
%      \figlab{test-2d-tc4-conv-tau-q}
%    }
%    \subfigure[$u_x$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-ux}
%      \figlab{test-2d-tc4-conv-tau-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-uy}
%      \figlab{test-2d-tc4-conv-tau-uy}
%    }
%%tau =1/h
%    \subfigure[$q$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-tau2-q}
%      \figlab{test-2d-tc4-conv-q}
%    }
%    \subfigure[$u_x$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-tau2-ux}
%      \figlab{test-2d-tc4-conv-ux}
%    }
%    \subfigure[$u_y$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-tau2-uy}
%      \figlab{test-2d-tc4-conv-uy}
%    }
%%tau=sqrt(phi)/h
%    \subfigure[$q$ with $\tau=\frac{\sqrt{\phi}}{h}$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-tau4-q}
%      \figlab{test-2d-tc4-conv-tau4-q}
%    }
%    \subfigure[$u_x$ with $\tau=\frac{\sqrt{\phi}}{h}$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-tau4-ux}
%      \figlab{test-2d-tc4-conv-tau4-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\frac{\sqrt{\phi}}{h}$]{
%      \includegraphics[trim=.1cm .1cm 2.2cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc4-conv-tau4-uy}
%      \figlab{test-2d-tc4-conv-tau4-uy}
%    }
%    \caption{Convergence study with different $\tau$ for the smooth solution test: scaled pressure $q$, scaled velocity component $u_x$ and scaled velocity component $u_y$ for $\tau=\sqrt{\phi}$, $\tau=1/h$ and $\tau=\sqrt{\phi}/h$. }
%    \figlab{test-2d-tc4-convergence}
%  \end{figure}
%
%
%\subsubsection{A non-smooth solution test in two dimensions}
%
%Figure \figref{test-2d-tc5a-convergece} shows the convergence study with $\beta=-1/4$. 
%
%
%
%\begin{figure}[h!t!b!]
%    \centering
%%tau=sqrt(phi)
%    \subfigure[$q$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-q}
%      \figlab{test-2d-tc5a-conv-q}
%    }
%    \subfigure[$u_x$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-ux}
%      \figlab{test-2d-tc5a-conv-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-uy}
%      \figlab{test-2d-tc5a-conv-uy}
%    }
%%tau=1/h
%    \subfigure[$q$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-tau2-q}
%      \figlab{test-2d-tc5a-conv-tau2-q}
%    }
%    \subfigure[$u_x$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-tau2-ux}
%      \figlab{test-2d-tc5a-conv-tau2-ux}
%    }
%    \subfigure[$u_y$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-tau2-uy}
%      \figlab{test-2d-tc5a-conv-tau2-uy}
%    }
%%tau=sqrt(\phi)/h
%    \subfigure[$q$ with $\tau=\sqrt{\phi}/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-tau4-q}
%      \figlab{test-2d-tc5a-conv-tau4-q}
%    }
%    \subfigure[$u_x$ with $\tau=\sqrt{\phi}/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-tau4-ux}
%      \figlab{test-2d-tc5a-conv-tau4-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\sqrt{\phi}/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5a-conv-tau4-uy}
%      \figlab{test-2d-tc5a-conv-tau4-uy}
%    }
%    \caption{Convergence study with different $\tau$ for the non-smooth solution test: scaled pressure $q$, scaled velocity component $u_x$ and scaled velocity component $u_y$ for $\tau=\sqrt{\phi}$, $\tau=1/h$ and $\tau=\sqrt{\phi}/h$. }
%    \figlab{test-2d-tc5a-convergece}
%  \end{figure}
%
%
%
%Figure \figref{test-2d-tc5b-convergece} shows the convergence study with $\beta=-3/4$. 
%
%\begin{figure}[h!t!b!]
%    \centering
%%tau=sqrt(phi)
%    \subfigure[$q$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-q}
%      \figlab{test-2d-tc5b-conv-q}
%    }
%    \subfigure[$u_x$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-ux}
%      \figlab{test-2d-tc5b-conv-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\sqrt{\phi}$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-uy}
%      \figlab{test-2d-tc5b-conv-uy}
%    }
%%tau=1/h
%    \subfigure[$q$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-tau2-q}
%      \figlab{test-2d-tc5b-conv-tau2-q}
%    }
%    \subfigure[$u_x$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-tau2-ux}
%      \figlab{test-2d-tc5b-conv-tau2-ux}
%    }
%    \subfigure[$u_y$ with $\tau=1/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-tau2-uy}
%      \figlab{test-2d-tc5b-conv-tau2-uy}
%    }
%%tau=sqrt(phi)/h
%    \subfigure[$q$ with $\tau=\sqrt{\phi}/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-tau4-q}
%      \figlab{test-2d-tc5b-conv-tau4-q}
%    }
%    \subfigure[$u_x$ with $\tau=\sqrt{\phi}/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-tau4-ux}
%      \figlab{test-2d-tc5b-conv-tau4-ux}
%    }
%    \subfigure[$u_y$ with $\tau=\sqrt{\phi}/h$]{
%      \includegraphics[trim=.1cm .1cm 1.0cm .1cm,clip=true,width=0.28\textwidth]{./figures/2d-tc5b-conv-tau4-uy}
%      \figlab{test-2d-tc5b-conv-tau4-uy}
%    }
%    \caption{Convergence study with different $\tau$ for the non-smooth solution test with $\beta=-3/4$: scaled pressure $q$, scaled velocity component $u_x$ and scaled velocity component $u_y$ for $\tau=\sqrt{\phi}$ and $\tau=1/h$.}
%    \figlab{test-2d-tc5b-convergece}
%  \end{figure}

